An OMNeT++ based Framework for Mobility-aware Routing in Mobile Robotic Networks

In this paper, we propose a cross-layer extension for the INETMANET framework of OMNeT++, which utilizes mobility control knowledge to enhance the forwarding of routing messages. The well-known mobility meta-model from Reynolds is used to provide a realistic representation of the mobility behavior of autonomous agents with respect to the various influences those agents have to face in real-world applications. Knowledge about the current mobility properties and its predicted development is used by mobility-aware routing mechanisms in order to optimize routing decisions and avoid path losses at runtime. In a proof of concept evaluation, we show that our proposed methods can achieve significant improvements to the robustness of communication paths.

==> tex/Abbreviations.tex <==
\addchap*{Abkürzungen} \label{cha:abbreviations}

% COMMAND OVERVIEW
%
% \ac{label}
% written out form at first usage, after this alway acronym
%
%  \acresetall
%  resets all acronyms to not used. Useful after the abstract to redefine all acronyms in the introduction.
%
%  \acf{label}
%  written out form with acronym in parentheses, irrespective of previous use
%
%  \acs{label}
%  acronym form, irrespective of previous use
%
%  \acl{label}
%  written out form without following acronym
%
%  \acp{label}
%  plural form of acronym by adding an s. \acfp. \acsp, \aclp work as well.


\begin{acronym}[E-UTRAN]  % Insert the abbrevation with most characters

%
% Please sort alphabetically!
%
\acro{16-QAM}{16 Quadrature Amplitude Modulation}
\acro{2G}{2nd Generation Mobile Networks}
\acro{3G}{3rd Generation Mobile Networks}
\acro{3GPP}{Third Generation Partnership Project}
\acro{3GPP2}{Third Generation Partnership Project 2}
\acro{3.5G}{3.5rd Generation Mobile Networks}
\acro{4G}{4th Generation Mobile Networks}
\acro{64-QAM}{64 Quadrature Amplitude Modulation}
\acro{AI}{Antenna Interface}
\acro{AMC}{Adaptive Modulation and Coding}
\acro{APN}{Access Point Name}
\acro{AQM}{Active Queue Management}
\acro{AWGN}{Additive White Guassian Noise}
\acro{BB}{Baseband}
\acro{BER}{Bit Error Rate}
\acro{BET}{Blind Equal Throughput}
\acro{BPSK}{Binary Phase Shift Keying}
\acro{BS}{Base Station}
\acro{BSE}{Base Station Emulator}
\acro{BSR}{Buffer Status Report}
\acro{CBR}{Constant Bit Rate}
\acro{CDMA}{Code Division Multiple Access}
\acro{CoPoMo}{Context-Aware Power Consumption Model for LTE User Equipment}
\acro{CP}{Cyclic Prefix}
\acro{CSG}{Closed Subscriber Group}
\acro{CQI}{Channel Quality Indicators}
\acro{CS}{Circuit Switched}
\acro{CSI}{Channel State Information}
\acro{DFT}{Discrete Fourier Transformation}
\acro{DL}{Downlink}
\acro{DLC}{Dynamic Link Classification}
\acro{DSL}{Digital Subscriber Line}
\acro{DVB-T}{Terrestiral Digital Video Broadcasting}
\acro{DwPTS}{Downlink Pilot Time Slot}
\acro{EARTH}{Energy Aware Radio and neTwork tecHnologies}
\acro{EASOS}{Energy Aware Switching-Off-Strategy}
\acro{eNB}{Evolved Node B}
\acro{EPC}{Evolved Packet Core}
\acro{EPS}{Evolved Packet System}
\acro{ETSI}{European Telecommunications Standards Institute}
\acro{E-UTRAN}{Evolved UMTS Terrestrial Radio Access Network}
\acro{FDD}{Frequency Division Duplex}
\acro{FDMA}{Frequency Division Multiple Access}
\acro{FEL}{Future Event List}
\acro{FFT}{Fast Fourier Transformation}
\acro{FIFO}{First In First Out}
\acro{FME}{First Maximum Expansion}
\acro{FPIA}{Fast Parameter Iteration Algorithmus} 
\acro{GGSN}{Gateway GPRS Support Node}
\acro{GP}{Guard Period}
\acro{GSM}{Global System for Mobile Communications}
\acro{GUI}{Graphical User Interface}
\acro{GW}{Gateway}
\acro{HSS}{Home Subscriber Server}
\acro{ICI}{Inter Carrier Interference}
\acro{IDFT}{Inverse Discrete Fourier Transformation}
\acro{IFFT}{Inverse Fast Fourier Transformation}
\acro{IKT}{Informations- und Kommunikationstechnologie}
\acro{IMT}{International Mobile Telecommunications}
\acro{IP}{Internet Protocol}
\acro{IPv4}{IP Version 4}
\acro{IPv6}{IP Version 6}
\acro{ISI}{Intersymbol Interference}
\acro{ITU}{International Telecommunication Union}
\acro{KA}{Keep Alive}
\acro{LTE}{Long Term Evolution}
\acro{M2M}{Machine-to-Machine}
\acro{MCS}{Modulation And Coding Scheme}
\acro{ME}{Mobile Equipment}
\acro{MIMO}{Multiple Input Multiple Output}
\acro{MLP}{Multi-Layer Perceptron}
\acro{MME}{Mobility Management Entity}
\acro{MT}{Maximum Throughput}
\acro{MTC}{Machine-Type Communication}
\acro{NGMN}{Next Generation Mobile Networks}
\acro{nrt}{Non Real Time}
\acro{PA}{Power Amplifier}
\acro{PAPR}{Peak to Average Power Ratio}
\acro{PDC}{Packet Data Core}
\acro{PDCCH}{Physical Downlink Control Channel}
\acro{PDN}{Packet Data Network}
\acro{PDR}{Packet Delivery Ratio}
\acro{PDSCH}{Physical Downlink Shared Channel}
\acro{PF}{Proportional Fair}
\acro{P-GW}{Packet Data Network Gateway}
\acro{PUCCH}{Physical Uplink Control Channel}
\acro{PUSCH}{Physical Uplink Shared Channel}
\acro{QCI}{QoS Class Identifier}
\acro{QoE}{Quality Of Experience}
\acro{QoS}{Quality of Service}
\acro{QPSK}{Quadrature Phase Shift Keying}
\acro{OFDM}{Orthogonal Frequency Division Multiplexing}
\acro{OFDMA}{Orthogonal Frequency Division Multiple Access}
\acro{RAN}{Radio Access Network}
\acro{RB}{Resource Block}
\acro{RE}{Resource Element}
\acro{RF}{Radio Frequency}
\acro{RR}{Round Robin}
\acro{RRH}{Remote Radio Head}
\acro{RRU}{Remote Radio Unit}
\acro{rt}{Real Time}
\acro{RNC}{Radio Network Controller}
\acro{RRM}{Radio Resource Management}
\acro{RSRP}{Referenz Signal Received Power}
\acro{RSRQ}{Reference Signal Received Quality}
\acro{RSSI}{Received Signal Strength Indication}
\acro{SAE}{System Architecture Evolution}
\acro{SDMA}{Space Division Multiple Access}
\acro{SC-FDMA}{Single Carrier Frequency Division Multiple Access}
\acro{SGSN}{Serving GPRS Support Node}
\acro{S-GW}{Serving Gateway}
\acro{SIM}{Subscriber Identity Module}
\acro{SINR}{Signal to Interference plus Noise Ratio}
\acro{SNR}{Signal to Noise Ratio}
\acro{SVM}{Support Vektor Maschine}
\acro{TA}{Timing Advance}
\acro{TBS}{Transport Block Size}
\acro{TDD}{Time Division Duplex}
\acro{TDMA}{Time Division Multiple Access}
\acro{TE}{Terminal Equipment}
\acro{TPC}{Transmission Power Control}
\acro{TRX}{Transceiver}
\acro{TTI}{Transmit Time Interval}
\acro{UDP}{User Datagram Protocol}
\acro{UE}{User Equipment}
\acro{UICC}{Universal Integrated Circuit Card}
\acro{UL}{Uplink}
\acro{ULPC}{Uplink Power Control}
\acro{UMTS}{Universal Mobile Telecommunications System}
\acro{USIM}{Universal Subscriber Identity Module}
\acro{UTRAN}{UMTS Terrestrial Radio Access Network}
\acro{UwPTS}{Uplink Pilot Time Slot}
\acro{VNI}{Visual Networking Index}
\acro{VoIP}{Voice Over IP}
\acro{VoLTE}{Voice Over LTE}
\acro{WEC}{World Energy Council}
\acro{WiMAX}{Worldwide Interoperability for Microwave Access}
\acro{WLAN}{Wireless Local Area Network}

%
% End of Acronym
%
\end{acronym}

%\ac{PTX}
\acresetall


==> tex/prediction_methods.tex <==

\renewcommand{\arraystretch}{1.1}
\begin{table}[h]
	\centering
	\caption{Properties of the prediction methods}
	\begin{tabular}{l|l|l|}
		\hline
		{\bf Parameter} 	& {\bf Remote Prediction}		& {\bf Local Prediction}                     		  \\ \hline
		

		Overhead & high & low \\ \hline
		Approach & Path Planning & Stigmergy \\ \hline
		Metric & Predictive Geo-based Dijkstra & Path Score \\ \hline
		

	\end{tabular}
	\label{tab:prediction_methods}
	\vspace{-10pt}
\end{table}

==> tex/statistics.tex <==
\subsection{Statistics}

\ac{PDR}
